Prior Based Online Lane Graph Extraction from Single Onboard Camera Image

The local road network information is essential for autonomous navigation. This information is commonly obtained from offline HD-Maps in terms of lane graphs. However, the local road network at a given moment can be drastically different than the one given in the offline maps; due to construction works, accidents etc. Moreover, the autonomous vehicle might be at a location not covered in the offline HD-Map. Thus, online estimation of the lane graph is crucial for widespread and reliable autonomous navigation. In this work, we tackle online Bird's-Eye-View lane graph extraction from a single onboard camera image. We propose to use prior information to increase quality of the estimations. The prior is extracted from the dataset through a transformer based Wasserstein Autoencoder. The autoencoder is then used to enhance the initial lane graph estimates. This is done through optimization of the latent space vector. The optimization encourages the lane graph estimation to be logical by discouraging it to diverge from the prior distribution. We test the method on two benchmark datasets, NuScenes and Argoverse. The results show that the proposed method significantly improves the performance compared to state-of-the-art methods.

==> experiments.tex <==


\section{Experiments}

We use the NuScenes \cite{nuscenes2019} and Argoverse \cite{DBLP:conf/cvpr/ChangLSSBHW0LRH19} datasets. The data processing and the train/test splits are the same as~\cite{Can_2021_ICCV}. 

\noindent\textbf{Implementation.}
The BEV area that our method outputs the lane graph is from -25 to 25m in x-direction and 1 to 50m in z direction with a 25cm resolution. We opt for using three Bezier control points. Our implementation is in Pytorch and runs with 7FPS. We set the latent space optimization loss trade-off parameter to $\alpha=0.02$. We run 600 iterations for the latent space optimization with a learning rate of 0.1. We use 32 helper vectors and 100 query vectors. The latent space of the WAE, and the hidden dimension of the transformer is 512. For the training of the WAE, $\beta=2$, $\gamma=1$ and $\theta=1$.


\noindent\textbf{Baselines.}
We compare against state-of-the-art~\textbf{transformer} and~\textbf{Polygon-RNN} based methods proposed in~\cite{Can_2021_ICCV} as well as another baseline which uses the method~\textbf{PINET}~\cite{DBLP:journals/corr/abs-2002-06604} to extract lane boundaries. We only train our method using the transformer based estimates. However, our method can be used in conjunction with any method.

\begin{figure*}
%\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=.9\linewidth]{figures/all_results.pdf}
    \vspace{-1em}
    \caption{The visual results from Nuscenes (top two rows) and Argoverse (bottom two rows). The visuals confirm that the proposed method produces more realistic and accurate lane graphs. The image level lane boundary estimates of PINET are projected onto the image.
    }
    \label{fig:results}
    \vspace{-1em}
%\end{subfigure}    
\end{figure*}

\noindent\textbf{Ablations.} We trained an autoencoder with the true lane graphs, refereed as \textbf{OursTrue}, instead of the proposed method where the autoencoder is trained with the estimated lane graphs (\textbf{Ours}), see Table~\ref{tab:nusc}. For both networks, we report the performance when no latent space optimization is carried out (\textbf{w/o Opt}) and when we apply latent space optimization. Moreover, we report the convergence behaviour of the latent space optimization for both the true lane graph trained network and ours (Fig.~\ref{fig:graphs}). 



